Table-To-Text generation and pre-training with TabT5

Encoder-only transformer models have been successfully applied to different table understanding tasks, as in TAPAS (Herzig et al., 2020). A major limitation of these architectures is that they are constrained to classification-like tasks such as cell selection or entailment detection. We present TABT5, an encoder-decoder model that generates natural language text based on tables and textual inputs. TABT5 overcomes the encoder-only limitation by incorporating a decoder component and leverages the input structure with table specific embeddings and pre-training. TABT5 achieves new state-of-the-art results on several domains, including spreadsheet formula prediction with a 15% increase in sequence accuracy, QA with a 2.5% increase in sequence accuracy and data-to-text generation with a 2.5% increase in BLEU.

==> tables.tex <==
\begin{table}[!h]
\caption{common caption for all tables}
    \begin{subtable}{0.5\textwidth}

\centering
\footnotesize
\begin{tabular}{@{}lS[table-format=2.2(1), separate-uncertainty, detect-weight]S[table-format=2.2(1), , separate-uncertainty, detect-weight]@{}} % centered columns
\toprule
\textbf{Model} & \textbf{Dev} & \textbf{Test} \\ [0.5ex] 
\midrule
\citeauthor{tapas}           & 85.1 & 83.6 \\
\citeauthor{min2019discrete} & 84.4 & 83.9 \\
T5-base  & 85.29(45) & 84.27(39)\\
\hline
\algo-small & 90.56(15) & 89.15(10) \\
\algo-large & 94.92(4) & 93.61(09) \\
\algo-base                   & \B 92.55(23) & \B 91.45(21) \\ %[1ex] % [1ex] adds vertical space
\Hquad + ToTTify  & 91.34(17) & 90.06(15)\\
\Hquad \textsc{-masking} & 88.87(31) & 87.51(19) \\
\Hquad \textsc{-embeddings} & 85.51(23) & 84.39(13)\\
\bottomrule
\end{tabular}
\caption{\wikisql{} denotation accuracy.} % title of Table
\label{table:wikisqlresults}
    
    \end{subtable}%
    \begin{subtable}{0.5\textwidth}
    
\centering
\footnotesize
\begin{tabular}{@{}lS[table-format=2.2(1), separate-uncertainty, detect-weight]@{}} % centered columns
\toprule

\textbf{Model} & \textbf{Top-1} \\%& \textbf{Top-5} & \textbf{Top-10} \\ [0.5ex] 
\midrule
\citeauthor{chen2021spreadsheetcoder} & 42.51\\% & 54.41 & 58.57 \\
\citeauthor{cheng2021fortap}          & 56.30 \\
T5-base & 69.40(33)\\
\hline
\algo-small & 71.33(24)\\
\algo-large & 71.79(20)\\
\algo-base & \B 71.61(27)\\
\Hquad + ToTTify & 71.18(22)\\
\Hquad \textsc{-masking} & 70.47(28)\\
\Hquad \textsc{-embeddings} & 70.07(36)\\
\bottomrule
\end{tabular}
\caption{\scoder{} accuracy.} % title of Table
\label{table:scoderresults-noformula}    

    \end{subtable}
\end{table}
    
\begin{table}[!h]
\caption{common caption for all tables}
    \begin{subtable}{1.0\textwidth}
    
\centering
\footnotesize
\begin{tabular}{@{}lS[table-format=2.2(1), separate-uncertainty, detect-weight]S[table-format=2.2(1), separate-uncertainty, detect-weight]S[table-format=2.2(1), separate-uncertainty, detect-weight]S[table-format=2.2(1), separate-uncertainty, detect-weight]@{}} % centered columns
  & \multicolumn{2}{c}{\emph{Overall}} & \multicolumn{2}{c}{\emph{Non-Overlap}} \\

\toprule
 \textbf{Model} & \textbf{BLEU} & \textbf{PARENT} & \textbf{BLEU} & \textbf{PARENT} \\
\midrule
\citeauthor{totto} & 44.00 & 52.60 & 35.10 & 46.80 \\
\citeauthor{kale2020text} & 47.70 & 57.10 & 39.50 & 52.60 \\
T5-base & 45.50(07) & 54.70(18) & 37.0(18) & 49.68(26) \\
\hline
\algo-small & 47.80(26) & 56.89(29) & 39.30(26) & 51.93(35)\\
\algo-base  & 49.00(07) & 57.70(11) & 40.90(13) & 53.12(18)\\
\Hquad + ToTTify & \B 49.50(07) & \B 57.95(05) & \B 41.60(05) & \B 53.65(07)\\
\Hquad \textsc{-masking} & 45.40(45) & 54.46(28) & 36.60(13) & 49.27(37) \\
\Hquad \textsc{-embeddings} & 48.60(17) & 57.12(23) & 40.50(26) & 52.71(28) \\
\bottomrule
\end{tabular}
	\caption{\totto{} results.}
	\label{table:tottoresults}
    
    \end{subtable}
\end{table}
